Faces that Speak: Jointly Synthesising Talking Face and Speech from Text

The goal of this work is to simultaneously generate natural talking faces and speech outputs from text. We achieve this by integrating Talking Face Generation (TFG) and Text-to-Speech (TTS) systems into a unified framework. We address the main challenges of each task: (1) generating a range of head poses representative of real-world scenarios, and (2) ensuring voice consistency despite variations in facial motion for the same identity. To tackle these issues, we introduce a motion sampler based on conditional flow matching, which is capable of high-quality motion code generation in an efficient way. Moreover, we introduce a novel conditioning method for the TTS system, which utilises motion-removed features from the TFG model to yield uniform speech outputs. Our extensive experiments demonstrate that our method effectively creates natural-looking talking faces and speech that accurately match the input text. To our knowledge, this is the first effort to build a multimodal synthesis system that can generalise to unseen identities.

==> tab/audio_mapper.tex <==
\begin{table}[!t]
    \centering
    \resizebox{0.95\linewidth}{!}
    {
        \renewcommand{\arraystretch}{1.3}
        \begin{tabular}{l|cc|c|c}
        \hline\hline
        \multirow{2}{*}{\bf Models} & \multicolumn{2}{|c}{\bf Video Quality} & \multicolumn{1}{|c}{\bf Synchonisation} & \multicolumn{1}{|c}{\bf Diversity} \\ 
        \cline{2-5}
         & {FID}$\downarrow$ & {ID-SIM}$\uparrow$\quad & {LSE-C}$\uparrow$\quad & {DIV}$\uparrow$\quad \\ 
        \hline
        1d-conv & 19.473 & 0.849 & 5.602 & 0.141 \\
        % 1d-conv (VoxCeleb2) & 0.000 & 0.858 & 5.622 & 0.138 \\
        MRF & \bf 18.348 & \bf 0.864 & \bf 5.686 & \bf 0.143 \\
        % MRF (VoxCeleb2) & 0.000 & 0.876 & 5.721 & 0.143 \\
        \hline\hline
        \end{tabular}
    }
\vspace{-1mm}
\caption{Design choice of audio mapper. These results are obtained on the LRS2 dataset using a one-shot generation setting.}
\label{tab:audio_mapper}
\end{table}


==> tab/cross_id_results.tex <==
\begin{table}[!t]
    \centering
    \resizebox{0.95\linewidth}{!}
    {
        \renewcommand{\arraystretch}{1.3}
        \begin{tabular}{l|cc|cc}
        \hline\hline
         & \multicolumn{2}{|c}{LRS2}  & \multicolumn{2}{|c}{LRS3} \\ 
        \cline{2-5}
        Method & {ID-SIM}$\downarrow$\quad & {LSE-C}$\uparrow$\quad &  {ID-SIM}$\downarrow$\quad & {LSE-C}$\uparrow$\quad \\ 
        \hline
        PC-AVS~\cite{zhou2021pose} & 0.00 & 0.00 & 0.00 & 0.00 \\
        PC-AVS (Cascade) & 0.00 & 0.00 & 0.00 & 0.00 \\
        FC-TFG~\cite{jang2023s} & 0.00 & 0.00 & 0.00 & 0.00 \\
        FC-TFG (Cascade) & 0.00 & 0.00 & 0.00 & 0.00 \\
        \hline
        Ours (Cascade) & 0.00 & 0.00 & 0.00 & 0.00 \\
        Ours & 0.00 & 0.00 & 0.00 & 0.00 \\
        \hline\hline
        \end{tabular}
    }
\caption{\textbf{Quantitative Results of Cross-id Generation.} }
\label{tab:cross_results}
\end{table}


==> tab/feature_analysis.tex <==
\begin{table}[!t]
    \centering
    \resizebox{0.85\linewidth}{!}
    {
        \centering
        \renewcommand{\arraystretch}{1.1}
        \begin{tabular}{c|ccccc}
        \hline\hline
        \multicolumn{1}{c|}{Orthogonal} & \multicolumn{5}{c}{Metrics} \\ 
        \cline{2-6}
        Constraint        & SSIM$\uparrow$ & MS-SSIM$\uparrow$ & PSNR$\uparrow$ & LMD$\downarrow$ & LSE-C$\uparrow$ \\ 
        \hline
        \xmark & 0.67 & 0.76 & 20.88 & 1.70 & 8.27 \\
        Cosine & 0.67 & 0.75 & 21 & 2.11 & 8.38 \\
        $L_{ortho}$ & \textbf{0.69} & \textbf{0.77} & \textbf{21.22} & \textbf{1.58} & \textbf{8.46} \\
        \hline\hline
        \end{tabular}
    }
\caption{.}
% \vspace{-2mm}
\label{tab:features}
\end{table}

==> tab/prior.tex <==
\begin{table}[!t]
    \centering
    \resizebox{0.95\linewidth}{!}
    {
        \renewcommand{\arraystretch}{1.3}
        \begin{tabular}{l|cc|c|c}
        \hline\hline
        \multirow{2}{*}{\bf Models} & \multicolumn{2}{|c}{\bf Video Quality} & \multicolumn{1}{|c}{\bf Synchonisation} & \multicolumn{1}{|c}{\bf Diversity} \\ 
        \cline{2-5}
         & {FID}$\downarrow$ & {ID-SIM}$\uparrow$\quad & {LSE-C}$\uparrow$\quad & {DIV}$\uparrow$\quad \\ 
        \hline
        LSTM & \bf 17.391 & \bf 0.870 & 5.578 & 0.140 \\
        % LSTM (VoxCeleb2)& 0.000 & 0.896 & 5.995 & 0.138 \\
        Conformer & 18.348 & 0.864 & \bf 5.686 & \bf 0.143 \\
        % Conformer (VoxCeleb2) & 0.000 & 0.876 & 5.721 & 0.143 \\
        \hline\hline
        \end{tabular}
    }
\caption{Design choice of prior network. These results are obtained on the LRS2 dataset using a one-shot generation setting.}
\label{tab:prior}
\end{table}

==> tab/rebuttal_cossim.tex <==
\begin{table}[!t]
    \centering
    \resizebox{0.50\linewidth}{!}
    {
        \renewcommand{\arraystretch}{1.0}
        \begin{tabular}{l|cc}
        \hline\hline
        {\bf Model} & {SIM} $\uparrow$ & {Std} $\downarrow$ \\ 
        \hline
        Face-TTS & 0.7768 & 0.027 \\
        Ours & \bf 0.8389 & \bf 0.024 \\
        \hline\hline
        \end{tabular}
    }
\vspace{-3mm}
\caption{The consistency of the generated voices.}
\vspace{-5mm}
\label{tab:consistency}
\end{table}


==> tab/sup_steps.tex <==
\begin{table}[!t]
    \centering
    \resizebox{0.95\linewidth}{!}
    {
        \renewcommand{\arraystretch}{1.3}
        \begin{tabular}{l|cc|c|c|c}
        \hline\hline
        \multirow{2}{*}{\bf Steps} & \multicolumn{2}{|c}{\bf Video Quality} & \multicolumn{1}{|c}{\bf Synchonisation} & \multicolumn{1}{|c}{\bf Diversity} & \multicolumn{1}{|c}{\bf Latency} \\ 
        \cline{2-6}
         & {FID}$\downarrow$ & {ID-SIM}$\uparrow$\quad & {LSE-C}$\uparrow$\quad & {DIV}$\uparrow$\quad & {Speed}$\uparrow$\quad\\ 
        \hline
        5 & \bf 18.384 & \bf 0.868 & \bf 5.801 & 0.132 & \bf 1,086 \\
        10 & 18.348 & 0.864 & 5.686 & 0.143 & 804\\
        50 & 18.645 & 0.857 & 5.548 & \bf 0.151 & 131\\
        \hline\hline
        \end{tabular}
    }
\vspace{-1mm}
\caption{Ablation on synthesis step of motion sampler. ``Speed" refers to the number of frames the module can handle per second. \emph{In other words, we measure the time consumed for mapping from audio and prior features to motion features.} These results are obtained on the LRS2 dataset using a one-shot generation setting.}
\label{tab:step}
\end{table}


==> tab/sup_tts_mos.tex <==
\begin{table}[!t]
    \centering
    \resizebox{0.9\linewidth}{!}
    {
        \renewcommand{\arraystretch}{1.3}
        \begin{tabular}{l|c|c}
        \hline\hline
        \multirow{2}{*}{\textbf{Models}} &\multicolumn{1}{c|}{\textbf{Naturalness}} &\multicolumn{1}{c}{\textbf{Voice similarity}} \\
        \cline{2-3}
         & {nMOS}$\uparrow$\quad &{sMOS}$\uparrow$\quad   \\ \hline
        Ground Truth &4.16$\pm$0.18 &4.96$\pm$0.03 \\ \hline
        Face-TTS  &2.57$\pm$0.15 & 2.18$\pm$0.14 \\ 
        Ours (w/ motion) &3.23$\pm$0.15& 2.45$\pm$0.16   \\ 
        Ours (w/o motion) &\textbf{3.49}$\pm$\textbf{0.15} & \textbf{2.94}$\pm$\textbf{0.16} \\ 
        \hline\hline
        \end{tabular}
    }
\vspace{-1mm}
\caption{MOS results of synthesised speech are presented with 95\% confidence interval. nMOS and sMOS represent naturalness and voice similarity, respectively. }
\label{tab:TTS_mos}
\end{table}


==> tab/target_results.tex <==
\begin{table*}[!t]
    \centering
    \resizebox{0.95\linewidth}{!}
    {
        \renewcommand{\arraystretch}{1.3}
        \begin{tabular}{l|ccccc|ccccc}
        \hline\hline
         & \multicolumn{5}{|c}{LRS2}  & \multicolumn{5}{|c}{LRS3} \\ 
        \cline{2-11}
        Method & {SSIM}$\uparrow$\quad & {MS-SSIM}$\uparrow$\quad & {PSNR}$\uparrow$\quad & {LMD}$\downarrow$\quad & {LSE-C}$\uparrow$\quad & {SSIM}$\uparrow$\quad & {MS-SSIM}$\uparrow$\quad & {PSNR}$\uparrow$\quad & {LMD}$\downarrow$\quad & {LSE-C}$\uparrow$\quad \\ 
        \hline
        PC-AVS~\cite{zhou2021pose} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
        PC-AVS (Cascade) & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
        FC-TFG~\cite{jang2023s} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
        FC-TFG (Cascade) & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
        \hline
        Ours (Cascade) & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
        Ours & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
        \hline\hline
        \end{tabular}
    }
\caption{\textbf{Quantitative Results of Target Motion-based Generation.} }
\label{tab:main_results}
\end{table*}


==> tab/tts_comparison_lrs3.tex <==
\begin{table}[!t]
    \centering
    \resizebox{0.9\linewidth}{!}
    {
        \renewcommand{\arraystretch}{1.3}
        \begin{tabular}{l|cccc}
        \hline\hline
        & \multicolumn{4}{c}{LRS3} \\ 
        \cline{2-5}
        Method & {MCD}$\downarrow$\quad &  {C-SIM}$\uparrow$\quad &{RMSE}$\downarrow$ & {EER}$\downarrow$\quad \\ 
        \hline
        % Ground truth&0.00 &-- &-- & \\ \hline
        Face-TTS~\cite{lee2023imaginary}  & 5.24 & 0.635 &42.47 & 16.00 \\ % &10.80 WER
        Ours (w/ motion)& 5.38 & 0.580 &38.52 & 14.67 \\ % 5.38 \pm 0.082 MCD / / 4.80 WER
        Ours (w/o motion) &\textbf{5.07}& \textbf{0.693} &\textbf{36.49} & ~~\textbf{8.33}\\ %5.073 \pm 0.083 MCD / 5.91 WER
        \hline\hline
        \end{tabular}
    }
\caption{\textbf{Quantitative Results of Synthesised Speech.} }
\end{table}

